A User Modeling Pipeline for Studying Polarized Political Events in Social Media

This paper presents a user modeling pipeline to analyze discussions and opinions shared on social media regarding polarized political events (e.g., public polls). The pipeline follows a four-step methodology. First, social media posts and users metadata are crawled. Second, a filtering mechanism is applied to filter spammers and bot users. As a third step, demographics information is extracted out of the valid users, namely gender, age, ethnicity and location information. Finally, the political polarity of the users with respect to the analyzed event is predicted. In the scope of this work, our proposed pipeline is applied to two referendum scenarios (independence of Catalonia in Spain and autonomy of Lombardy in Italy) in order to assess the performance of the approach with respect to the capability of collecting correct insights on the demographics of social media users and of predicting the poll results based on the opinions shared by the users. Experiments show that the method was effective in predicting the political trends for the Catalonia case, but not for the Lombardy case. Among the various motivations for this, we noticed that in general Twitter was more representative of the users opposing the referendum than the ones in favor.

==> all_old_tables.tex <==
% \begin{figure}[t!]
%     \begin{subfigure}[t]{0.47\textwidth}t        \includegraphics[clip, trim=0cm 0cm 0cm 0cm, width=1.00\textwidth]{images/catalonia_eth_general.png}
%         \caption{Catalonia Referendum}
%         \label{fig:catalonia_eth_general}
%     \end{subfigure}    \hspace{1em}
%     \begin{subfigure}[t]{0.47\textwidth}
%         \includegraphics[clip, trim=0cm 0cm 0cm 0cm, width=1.00\textwidth]{images/lombardy_eth_general.png}
%         \caption{Lombardy Referendum}
%         \label{fig:lombardy_eth_general}
%     \end{subfigure}    \hspace{1em}
%     \caption{Distribution of users by ethnicity.}
%     \label{fig:eth_general}
% \end{figure}


% \begin{table}[]
% \centering
% \label{table:age}
% \begin{tabular}{@{}llccccccccc@{}}
% \toprule
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \textless 18 &  & 18 - 30 &  & 31 - 45 &  & 46 - 65 &  & \textgreater 65 \\ \midrule
% Catalonia &  & 4.9\% &  & 22.1\% &  & 41.0\% &  & 29.4\% &  & 2.6\% \\
% Lombardy &  & 5.5\% &  & 24.3\% &  & 37.6\% &  & 30.0\% &  & 2.6\% \\ \bottomrule
% \end{tabular}
% \caption{Classification of users by age.}
% \end{table}


%The results of the application of the user modeling pipeline are reported in the following tables. \\
%Table \ref{table:outliers} shows that across the two scenarios there are between 10\% and 15\% accounts that exhibited a greater post activity than normal users. These users were removed and will not be considered in the following analyses.

% outliers table
% \begin{table}
% \centering
% \caption{Number of valid users after the outlier analysis.}
% \label{table:outliers}
% \begin{tabular}{@{}lcccccccc@{}} 
% \toprule
%   & \textbf{Q1} & \textbf{Q2} & \textbf{Q3} & \textbf{IQR} & \textbf{Lower-Bound} & \textbf{Upper-Bound} & \textbf{Valid Users} & \textbf{Total Users} \\ 
% \midrule
%   \textbf{Catalonia} & 24.81 & 92.51 &	298.35 & 273.53 & -385.49 & 708.65 & 1376375 & 1548745 \\
%   \textbf{Lombardia} & 26.82 & 103.08 & 372.31 & 345.49 & -491.42 & 890.55 & 22375 & 25487 \\
% \bottomrule
% \end{tabular}
% \end{table}

%Table \ref{table:bots} shows the number of users classified as bots. Both scenarios were characterized by a high number of bot accounts, since more than half of the users were classified as such (52\% for the Lombardy case, 58\% for the Catalonia case). The English-independent score is abbreviated as UNI, while the English-dependent score is abbreviated as ENG. The users selected for the following analyses are only those with a universal score < 40.

% bot table
% \begin{table}
% \centering
% \caption{Number of valid users after the bot analysis.}
% \label{table:bots}
% \begin{tabular}{@{}lccccc@{}} 
% \toprule
%   & UNI \textless 40 & \textbf{UNI \textless 50} & \textbf{ENG \textless 40} & \textbf{ENG \textless 50} & \textbf{Total Users} \\ 
% \midrule
%   \textbf{Catalonia} & 530318 & 582039 & 487932 & 577071 & 1376375 \\
%   \textbf{Lombardia} & 9284 & 10801 & 8652 & 10819 & 22375 \\
% \bottomrule
% \end{tabular}
% \end{table}

%\subsubsection
% The following tables summarize the demographics findings of the users. Table \ref{table:gender}, Table \ref{table:age} and Table \ref{table:ethn cat}, Table \ref{table:ethn lomb} sum up the results for gender, age and ethnicity analysis respectively.

% gender table
% \begin{table}[]
% \centering
% \caption{Classification of users by gender.}
% \label{table:gender}
% \begin{tabular}{@{}lcccc@{}}
% \toprule
%  & Female & Male & Unclassified & Total \\ 
% \midrule
% Catalonia & 168791 & 296840 & 116408 & 582039 \\
% Lombardia & 2546 & 5088 & 3167 & 10801 \\ 
% \bottomrule
% \end{tabular}
% \end{table}

% age table
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c|c| } 
%  \hline
%   & \textbf{\textless 18} & \textbf{18 - 30} & \textbf{31 - 45} & \textbf{46 - 65} & \textbf{\textgreater 65} & \textbf{Unclassified} & \textbf{Total Users} \\ 
%  \hline
%   \textbf{Catalonia} & 11404 & 51468 & 95381 & 68470 & 6072 & 349244 & 582039 \\
%   \hline
%   \textbf{Lombardia} & 270	 & 1175 & 1819 & 1451 & 126 & 5960 & 10801 \\
%  \hline
% \end{tabular}
% \caption{Classification of users by age.}
% \label{table:age}
% \end{center}
% \end{table}

% ethnicities table
% \begin{table}
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{ |c|c| } 
%  \hline
%  \textbf{Ethnicity} & \textbf{\# Users} \\ 
%  \hline
%   \textbf{Hispanic} & 103277 \\
%   \hline
%   \textbf{British} & 83064 \\
%   \hline
%   \textbf{White} & 63602 \\
%   \hline
%   \textbf{Italian} & 51797 \\
%   \hline
%   \textbf{Indian Subcontinent} & 35078 \\
%   \hline
%   \textbf{French} & 30865 \\
%   \hline
%   \textbf{Jewish} & 27309 \\
%   \hline
%   \textbf{Africans} & 25752 \\
%   \hline
%   \textbf{Muslim} & 24073 \\
%   \hline
%   \textbf{East European} & 22054 \\
%   \hline
%   \textbf{Japanese} & 15928 \\
%   \hline
%   \textbf{East Asian} & 14208 \\
%   \hline
%   \textbf{Germanic} & 9773 \\
%   \hline
%   \textbf{Nordic} & 9397 \\
%   \hline
%   \textbf{Asian} & 8439 \\
%   \hline
%   \textbf{Black} & 3760 \\
%   \hline
%   \textbf{Undefined} & 53663 \\
%   \hline
%   \textbf{Total Users} & 582039 \\
%  \hline
% \end{tabular}
% \caption{Classification of users by ethnicity for the Catalonia scenario.}
% \label{table:ethn cat}
% }
% \hfill
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{ |c|c| } 
%  \hline
%  \textbf{Ethnicity} & \textbf{\# Users} \\ 
%  \hline
%   \textbf{White} & 3228 \\
%   \hline
%   \textbf{Italian} & 1887 \\
%   \hline
%   \textbf{British} & 552 \\
%   \hline
%   \textbf{Hispanic} & 427 \\
%   \hline
%   \textbf{Asian} & 319 \\
%   \hline
%   \textbf{French} & 234 \\
%   \hline
%   \textbf{Indian Subcontinent} & 235 \\
%   \hline
%   \textbf{Jewish} & 226 \\
%   \hline
%   \textbf{Africans} & 221 \\
%   \hline
%   \textbf{Muslim} & 205 \\
%   \hline
%   \textbf{East European} & 188 \\
%   \hline
%   \textbf{Black} & 129 \\
%   \hline
%   \textbf{Japanese} & 118 \\
%   \hline
%   \textbf{East Asian} & 111 \\  
%   \hline
%   \textbf{Nordic} & 78 \\
%   \hline
%   \textbf{Germanic} & 72 \\    
%   \hline
%   \textbf{Undefined} & 2571 \\
%   \hline
%   \textbf{Total Users} & 10801 \\
%  \hline
% \end{tabular}
% \caption{Classification of users by ethnicity for the Lombardia scenario.}
% \label{table:ethn lomb}
% }
% \end{table}

%\subsubsection
%Table \ref{table:cntr cat}, Table \ref{table:cntr lomb}, Table \ref{table:reg cat}, Table \ref{table:reg lomb} and Table \ref{table:city cat}, Table \ref{table:city lomb} sum up the results of the location analysis.

% countries table
% \begin{table}
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{ |c|c| } 
%  \hline
%  \textbf{Country} & \textbf{\# Users} \\ 
%  \hline
%   \textbf{ES} & 79023 \\
%   \hline
%   \textbf{US} & 15568 \\
%   \hline
%   \textbf{GB} & 13890 \\
%   \hline
%   \textbf{FR} & 4943 \\
%   \hline
%   \textbf{IT} & 3074 \\
%   \hline
%   \textbf{NL} & 1551 \\
%   \hline
%   \textbf{DE} & 1395 \\
%   \hline
%   \textbf{IE} & 1363 \\  
%   \hline
%   \textbf{BE} & 944 \\
%   \hline
%   \textbf{AT} & 180 \\
%   \hline
% \end{tabular}
% \caption{10 countries with the greatest number of users for the Catalonia scenario.}
% \label{table:cntr cat}
% }
% \hfill
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{ |c|c| } 
%  \hline
%  \textbf{Country} & \textbf{\# Users} \\ 
%  \hline
%   \textbf{IT} & 4744 \\
%   \hline
%   \textbf{ES} & 243 \\
%   \hline
%   \textbf{US} & 153 \\
%   \hline
%   \textbf{BR} & 146 \\
%   \hline
%   \textbf{GB} & 113 \\
%   \hline
%   \textbf{FR} & 53 \\
%   \hline
%   \textbf{AR} & 49 \\  
%   \hline
%   \textbf{NL} & 35 \\
%   \hline
%   \textbf{BE} & 34 \\
%   \hline
%   \textbf{DE} & 31 \\
%  \hline
% \end{tabular}
% \caption{10 countries with the greatest number of users for the Lombardia scenario.}
% \label{table:cntr lomb}
% }
% \end{table}

% regions table
% \begin{table}
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{ |c|c| } 
%  \hline
%  \textbf{Region} & \textbf{\# Users} \\ 
%  \hline
%  \textbf{Andalusia} & 7373 \\
%   \hline
%   \textbf{Catalonia} & 11503 \\
%   \hline
%   \textbf{Community of Madrid} & 9795 \\
%   \hline
%   \textbf{Valencian Community} & 3668 \\
%   \hline
%   \textbf{Galicia} & 1752 \\
%   \hline
%   \textbf{Castille and León} & 1711 \\  
%   \hline
%   \textbf{Basque Country} & 1387 \\
%   \hline
%   \textbf{Castilla-La Mancha} & 1100 \\
%   \hline
%   \textbf{Canary Islands} & 1391 \\
%   \hline
%   \textbf{Region of Murcia} & 1146 \\
%   \hline  
% \end{tabular}
% \caption{10 regions with the greatest number of users for the Catalonia scenario.}
% \label{table:reg cat}
% }
% \hfill
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{ |c|c| } 
%  \hline
%  \textbf{Region} & \textbf{\# Users} \\ 
%  \hline
%   \textbf{Lombardy} & 1300 \\
%   \hline
%   \textbf{Veneto} & 799 \\
%   \hline
%   \textbf{Latium} & 553 \\
%   \hline
%   \textbf{Emilia-Romagna} & 197 \\
%   \hline
%   \textbf{Tuscany} & 145 \\
%   \hline
%   \textbf{Piedmont} & 132 \\
%   \hline
%   \textbf{Campania} & 130 \\  
%   \hline
%   \textbf{Apulia} & 103 \\
%   \hline
%   \textbf{Sicily} & 100 \\
%   \hline
%   \textbf{Friuli Venezia Giulia} & 83 \\
%  \hline
% \end{tabular}
% \caption{10 regions with the greatest number of users for the Lombardia scenario.}
% \label{table:reg lomb}
% }
% \end{table}

% cities table
% \begin{table}
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{ |c|c| } 
%  \hline
%  \textbf{City} & \textbf{\# Users} \\ 
%  \hline
%   \textbf{Madrid} & 10987 \\
%   \hline
%   \textbf{Barcelona} & 9591 \\
%   \hline
%   \textbf{Seville} & 2923 \\
%   \hline
%   \textbf{Valencia} & 2158 \\  
%   \hline
%   \textbf{Córdoba} &  \\
%   \hline
%   \textbf{Málaga} & 1557 \\
%   \hline
%   \textbf{Granada} &  \\
%   \hline
%   \textbf{Murcia} &  \\
%   \hline
%   \textbf{Bilbao} &  \\
%   \hline
%   \textbf{Zaragoza} &  \\
%   \hline  
% \end{tabular}
% \caption{10 cities with the greatest number of users for the Catalonia scenario.}
% \label{table:city cat}
% }
% \hfill
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{ |c|c| } 
%  \hline
%  \textbf{City} & \textbf{\# Users} \\ 
%  \hline
%   \textbf{Milan} & 1300 \\
%   \hline
%   \textbf{Rome} & 799 \\
%   \hline
%   \textbf{Venice} & 553 \\
%   \hline
%   \textbf{Padua} & 197 \\
%   \hline
%   \textbf{Verona} & 145 \\
%   \hline
%   \textbf{Turin} & 132 \\
%   \hline
%   \textbf{Vicenza} & 130 \\  
%   \hline
%   \textbf{Treviso} & 103 \\
%   \hline
%   \textbf{Naples} & 100 \\
%   \hline
%   \textbf{Bologna} & 83 \\
%  \hline
% \end{tabular}
% \caption{10 cities with the greatest number of users for the Lombardy scenario.}
% \label{table:city lomb}
% }
% \end{table}


% predictors performance tables
% relevance predictor
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c| } 
%  \hline
%   & & \textbf{Precision} & \textbf{Recall} & \textbf{F-Measure} & \textbf{Accuracy} \\ 
%  \hline
%  \multirow{2}{4em}{Catalonia} &  \textbf{Training} & 0.899 (+/- 0.008) & 0.901 (+/- 0.007) & 0.900 (+/- 0.005) & 0.900 (+/- 0.005) \\
%   \hline
%   & \textbf{Test} & 0.874 (+/- 0.043) & 0.863 (+/- 0.048) & 0.868 (+/- 0.018) & 0.869 (+/- 0.016) \\
%  \hline
%  \multirow{2}{4em}{Lombardy} & \textbf{Training} & 0.869 (+/- 0.007) & 0.950 (+/- 0.006) & 0.908 (+/- 0.004) & 0.904 (+/- 0.005) \\
%   \hline
%   & \textbf{Test} & 0.876 (+/- 0.025) & 0.946 (+/- 0.035) & 0.910 (+/- 0.020)	 & 0.905 (+/- 0.023) \\
%  \hline
% \end{tabular}
% \caption{Performance of the relevance predictor.}
% \label{table:rel pred perf}
% \end{center}
% \end{table}

% negative predictor
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c| } 
%  \hline
%   & & \textbf{Precision} & \textbf{Recall} & \textbf{F-Measure} & \textbf{Accuracy} \\ 
%   \hline
%  \multirow{2}{2em}{Catalonia} &  \textbf{Training} & 0.847 (+/- 0.019) & 0.860 (+/- 0.011) & 0.853 (+/- 0.013) & 0.852 (+/- 0.014) \\
%   \hline
%   & \textbf{Test} & 0.755 (+/- 0.062) & 0.799 (+/- 0.087) & 0.775 (+/- 0.045) & 0.773 (+/- 0.041) \\
%  \hline
%   \multirow{2}{2em}{Lombardy} & \textbf{Training} & 0.705 (+/- 0.016) & 0.722 (+/- 0.047) & 0.713 (+/- 0.023) & 0.712 (+/- 0.011) \\
%   \hline
%   & \textbf{Test} & 0.715 (+/- 0.076) & 0.713 (+/- 0.090) & 0.712 (+/- 0.035) & 0.706 (+/- 0.027) \\
%  \hline
% \end{tabular}
% \caption{Performance of the negative predictor.}
% \label{table:neg pred perf}
% \end{center}
% \end{table}

% positive predictor
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c| } 
%  \hline
%   & \textbf{Precision} & \textbf{Recall} & \textbf{F-Measure} & \textbf{Accuracy} \\ 
%   \hline
%  \multirow{2}{4em}{Catalonia} &  \textbf{Training} & 0.844 (+/- 0.027) & 0.833 (+/- 0.028) & 0.839 (+/- 0.022) & 0.839 (+/- 0.022) \\
%   \hline
%   & \textbf{Test} & 0.774 (+/- 0.055) & 0.759 (+/- 0.100) & 0.765 (+/- 0.052) & 0.770 (+/- 0.039) \\
%  \hline
%   \multirow{2}{4em}{Lombardy} & \textbf{Training} & 0.745 (+/- 0.016) & 0.785 (+/- 0.028) & 0.765 (+/- 0.019) & 0.758 (+/- 0.011) \\
%   \hline
%   & \textbf{Test} & 0.738 (+/- 0.070) & 0.789 (+/- 0.083) & 0.761 (+/- 0.042)	 & 0.756 (+/- 0.038) \\
%  \hline
% \end{tabular}
% \caption{Performance of the positive predictor.}
% \label{table:pos pred perf}
% \end{center}
% \end{table}


% polarization users
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%  \textbf{Positive} & \textbf{Negative} & \textbf{Neutral} & \textbf{Total Classified} & \textbf{Total Users} \\ 
%  \hline
%  1767 & 2368 & 2042 & 6177 & 10801 \\
%  \hline
% \end{tabular}
% \caption{Polarized users in the Lombardy users.}
% \label{table:pol users}
% \end{center}
% \end{table}


% Lombardia

% gender + political
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%   & \textbf{Female} & \textbf{Male} & \textbf{Total Classified} \\ 
%  \hline
%   \textbf{Yes} & 361 & 801 & 1162 \\
%   \hline
%   \textbf{No} & 550 & 1272 & 1822 \\
%   \hline
%   \textbf{Neutral} & 440 & 983 & 1423 \\
%   \hline
%   \textbf{Total} & 1351 & 3056 & 4407 \\
%  \hline
% \end{tabular}
% \caption{Classification of users by gender and political view for the Lombardy scenario.}
% \label{table:gender polit}
% \end{center}
% \end{table}

% % age + political
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c|c| } 
%  \hline
%   & \textbf{\textless 18} & \textbf{18 - 30} & \textbf{31 - 45} & \textbf{46 - 65} & \textbf{\textgreater 65} & \textbf{Total Classified} \\ 
%  \hline
%   \textbf{Yes} & 36 & 172 & 287 & 216 & 17 & 728 \\
%   \hline
%   \textbf{No} & 62 & 263 & 465 & 364 & 32 & 1186 \\
%   \hline
%   \textbf{Neutral} & 42 & 238 & 358 & 287 & 27 & 952 \\
%   \hline
%   \textbf{Total} & 140 & 673 & 1110 & 867 & 76 & 2866 \\
%  \hline
% \end{tabular}
% \caption{Classification of users by age and political view for the Lombardy scenario.}
% \label{table:age polit}
% \end{center}
% \end{table}

% % age + political + females
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c|c| } 
%  \hline
%   & \textbf{\textless 18} & \textbf{18 - 30} & \textbf{31 - 45} & \textbf{46 - 65} & \textbf{\textgreater 65} & \textbf{Total Classified} \\ 
%  \hline
%   \textbf{Yes} & 24 & 69 & 62 & 37 & 1 & 193 \\
%   \hline
%   \textbf{No} & 34 & 98 & 108 & 59 & 9 & 308 \\
%   \hline
%   \textbf{Neutral} & 18 & 94 & 69 & 56 & 4 & 241 \\
%   \hline
%   \textbf{Total} & 76 & 251 & 239 & 154 & 14 & 734 \\
%  \hline
% \end{tabular}
% \caption{Classification of users by age, female gender and political view for the Lombardy scenario.}
% \label{table:age fem polit}
% \end{center}
% \end{table}

% % age + political + males
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c|c| } 
%  \hline
%   & \textbf{\textless 18} & \textbf{18 - 30} & \textbf{31 - 45} & \textbf{46 - 65} & \textbf{\textgreater 65} & \textbf{Total Classified} & \textbf{Unclassified} \\ 
%  \hline
%   \textbf{Yes} & 10 & 102 & 215 & 169 & 15 & 511 \\
%   \hline
%   \textbf{No} & 28 & 158 & 346 & 272 & 21 & 825 \\
%   \hline
%   \textbf{Neutral} & 23 & 141 & 270 & 209 & 19 & 662 \\
%   \hline
%   \textbf{Total} & 61 & 401 & 831 & 650 & 55 & 1998 \\
%  \hline
% \end{tabular}
% \caption{Classification of users by age, male gender and political view for the Lombardy scenario.}
% \label{table:age male polit}
% \end{center}
% \end{table}

% % ethnicity + political
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%  \textbf{Ethnicity} & \textbf{Yes} & \textbf{No} & \textbf{Neutral} & \textbf{Total}  \\ 
%  \hline
%   \textbf{White} & 521 & 772 & 637 & 1930 \\
%   \hline
%   \textbf{Italian} & 343 & 445 & 367 & 1155 \\
%   \hline
%   \textbf{British} & 75 & 95 & 103 & 273 \\
%   \hline
%   \textbf{Hispanic} & 77 & 81 & 96 & 254 \\
%   \hline
%   \textbf{Asian} & 40 & 81 & 58 & 179 \\
%   \hline
%   \textbf{French} & 42 & 50 & 38 & 130 \\
%   \hline
%   \textbf{Indian Subcontinent} & 27 & 47 & 36 & 110 \\
%   \hline
%   \textbf{Jewish} & 35 & 35 & 48 & 118 \\
%   \hline
%   \textbf{Africans} & 37 & 46 & 34 & 117 \\
%   \hline
%   \textbf{Muslim} & 26 & 35 & 33 & 94 \\
%   \hline
%   \textbf{East European} & 35 & 36 & 41 & 112 \\
%   \hline
%   \textbf{Black} & 14 & 38 & 31 & 83 \\
%   \hline
%   \textbf{Japanese} & 11 & 27 & 32 & 70 \\
%   \hline
%   \textbf{East Asian} & 21 & 22 & 24 & 67 \\  
%   \hline
%   \textbf{Nordic} & 14 & 13 & 17 & 44 \\
%   \hline
%   \textbf{Germanic} & 14 & 18 & 9 & 41 \\   
%   \hline
%   \textbf{Total Users} & 1332 & 1841 & 1604 & 4777 \\
%  \hline
% \end{tabular}
% \caption{Classification of users by ethnicity and political view for the Lombardy scenario.}
% \label{table:ethn pol}
% \end{center}
% \end{table}


% % countries + political
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%  \textbf{Country} & \textbf{Yes} & \textbf{No} & \textbf{Neutral} & \textbf{Total} \\ 
%  \hline
%   \textbf{IT} & 31.32 & 37.74 & 30.94 \\
%   \hline
%   \textbf{ES} & 19.80 & 6.93 & 73.27  \\
%   \hline
%   \textbf{US} & 15.91 & 50.00 & 34.09  \\
%   \hline
%   \textbf{BR} & 6.67 & 33.33 & 60.00  \\
%   \hline
%   \textbf{GB} & 12.50 & 40.63 & 46.88 \\
%   \hline
%   \textbf{FR} & 21.74 & 39.13 & 39.13 \\
%   \hline
%   \textbf{AR} & 8.33 & 8.33 & 83.34 & 12  \\  
%   \hline
%   \textbf{NL} & 12.50 & 12.50 & 75.00 \\
%   \hline
%   \textbf{BE} & 22.73 & 31.82 & 45.46  \\
%   \hline
%   \textbf{DE} & 10.00 & 70.00 & 20.00  \\
%  \hline
% \end{tabular}
% \caption{10 countries with the greatest number of polarized users for the Lombardy scenario.}
% \label{table:cntr pol}
% \end{center}
% \end{table}

% % regions + political
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%  \textbf{Region} & \textbf{Yes} & \textbf{No} & \textbf{Neutral} & \textbf{Total} \\ 
%  \hline
%   \textbf{Lombardy} & 34.20 & 33.68 & 32.12 \\
%   \hline
%   \textbf{Veneto} & 29.68 & 37.40 & 32.93 \\
%   \hline
%   \textbf{Latium} & 32.21 & 36.98 & 30.81 \\
%   \hline
%   \textbf{Emilia-Romagna} & 28.57 & 40.48 & 30.95 \\
%   \hline
%   \textbf{Tuscany} & 36.90 & 42.86 & 20.24 \\
%   \hline
%   \textbf{Piedmont} & 34.21 & 38.16 & 27.63 \\
%   \hline
%   \textbf{Campania} & 23.91 & 52.17 & 23.91 \\  
%   \hline
%   \textbf{Apulia} & 41.67 & 45.00 & 13.33 \\
%   \hline
%   \textbf{Sicily} & 15.63 & 71.88 & 12.50 \\
%   \hline
%   \textbf{Friuli Venezia Giulia} & 21.28 & 40.43 & 38.30 \\
%  \hline
% \end{tabular}
% \caption{10 regions with the greatest number of polarized users for the Lombardy scenario.}
% \label{table:reg pol}
% \end{center}
% \end{table}

% % cities + political
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%  \textbf{City} & \textbf{Yes} & \textbf{No} & \textbf{Neutral} & \textbf{Total} \\ 
%  \hline
%  \textbf{Milan} & 33.11 & 36.26 & 30.63 \\
%   \hline
%   \textbf{Rome} & 31.02 & 37.95 & 31.02 \\
%   \hline
%   \textbf{Venice} & 38.27 & 29.63 & 32.10 \\
%   \hline
%   \textbf{Padua} & 28.10 & 40.45 & 31.46 \\
%   \hline
%   \textbf{Verona} & 22.64 & 41.51 & 35.85 \\
%   \hline
%   \textbf{Turin} & 22.73 & 47.73 & 29.55 \\
%   \hline
%   \textbf{Vicenza} & 21.74 & 43.48 & 34.78 \\  
%   \hline
%   \textbf{Treviso} & 29.73 & 29.73 & 40.54 \\
%   \hline
%   \textbf{Naples} & 26.53 & 53.06 & 20.41 \\
%   \hline
%   \textbf{Bologna} & 25.64 & 35.90 & 38.46 \\
%  \hline
% \end{tabular}
% \caption{10 cities with the greatest number of polarized users for the Lombardy scenario.}
% \label{table:city pol}
% \end{center}
% \end{table}



% Catalonia

% gender + political
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%   & \textbf{Female} & \textbf{Male} & \textbf{Total Classified} \\ 
%  \hline
%   \textbf{Yes} & 1139 & 2613 & 3770 \\
%   \hline
%   \textbf{No} & 1849 & 4376 & 6225 \\
%   \hline
%   \textbf{Neutral} & 1140 & 2815 & 3955 \\
%   \hline
%   \textbf{Total} & 4128 & 9804 & 13950 \\
%  \hline
% \end{tabular}
% \caption{Classification of users by gender and political view for the Catalonia scenario.}
% \label{table:gender polit}
% \end{center}
% \end{table}

% % age + political
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c|c| } 
%  \hline
%   & \textbf{\textless 18} & \textbf{18 - 30} & \textbf{31 - 45} & \textbf{46 - 65} & \textbf{\textgreater 65} & \textbf{Total Classified} \\ 
%  \hline
%   \textbf{Yes} & 128 & 671 & 1418 & 1178 & 114 & 3509 \\
%   \hline
%   \textbf{No} & 391 & 1460 & 2366 & 1496 & 96 & 5809 \\
%   \hline
%   \textbf{Neutral} & 180 & 856 & 1490 & 1102 & 82 & 3710 \\
%   \hline
%   \textbf{Total} & 699 & 2987 & 5274 & 3776 & 292 & 13028 \\
%  \hline
% \end{tabular}
% \caption{Classification of users by age and political view for the Catalonia scenario.}
% \label{table:age polit}
% \end{center}
% \end{table}

% % age + political + females
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c|c| } 
%  \hline
%   & \textbf{\textless 18} & \textbf{18 - 30} & \textbf{31 - 45} & \textbf{46 - 65} & \textbf{\textgreater 65} & \textbf{Total Classified} \\ 
%  \hline
%   \textbf{Yes} & 64 & 278 & 416 & 295 & 18 & 1071 \\
%   \hline
%   \textbf{No} & 220 & 535 & 623 & 330 & 12 & 1720 \\
%   \hline
%   \textbf{Neutral} & 102 & 297 & 407 & 259 & 6 & 1071 \\
%   \hline
%   \textbf{Total} & 386 & 1110 & 1446 & 884 & 36 & 3862 \\
%  \hline
% \end{tabular}
% \caption{Classification of users by age, female gender and political view for the Catalonia scenario.}
% \label{table:age fem polit}
% \end{center}
% \end{table}

% % age + political + males
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c|c| } 
%  \hline
%   & \textbf{\textless 18} & \textbf{18 - 30} & \textbf{31 - 45} & \textbf{46 - 65} & \textbf{\textgreater 65} & \textbf{Total Classified} & \textbf{Unclassified} \\ 
%  \hline
%   \textbf{Yes} & 64 & 393 & 1002 & 882 & 95 & 2436 \\
%   \hline
%   \textbf{No} & 171 & 925 & 1737 & 1162 & 84 & 4079 \\
%   \hline
%   \textbf{Neutral} & 78 & 558 & 1083 & 843 & 76 & 2638 \\
%   \hline
%   \textbf{Total} & 313 & 1876 & 3822 & 2887 & 255 & 9153 \\
%  \hline
% \end{tabular}
% \caption{Classification of users by age, male gender and political view for the Catalonia scenario.}
% \label{table:age male polit}
% \end{center}
% \end{table}

% % ethnicity + political
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%  \textbf{Ethnicity} & \textbf{Yes} & \textbf{No} & \textbf{Neutral} & \textbf{Total}  \\ 
%  \hline
%   \textbf{White} & 1574 & 3114 & 1730 & 6418 \\
%   \hline
%   \textbf{Italian} & 251 & 295 & 190 & 736 \\
%   \hline
%   \textbf{British} & 589 & 292 & 515 & 1396 \\
%   \hline
%   \textbf{Hispanic} & 429 & 1197 & 479 & 2105 \\
%   \hline
%   \textbf{Asian} & 124 & 308 & 200 & 632 \\
%   \hline
%   \textbf{French} & 158 & 186 & 148 & 492 \\
%   \hline
%   \textbf{Indian Subcontinent} & 110 & 159 & 161 & 430 \\
%   \hline
%   \textbf{Jewish} & 135 & 161 & 113 & 409 \\
%   \hline
%   \textbf{Africans} & 111 & 149 & 86 & 346 \\
%   \hline
%   \textbf{Muslim} & 106 & 128 & 118 & 352 \\
%   \hline
%   \textbf{East European} & 100 & 142 & 83 & 325 \\
%   \hline
%   \textbf{Black} & 82 & 133 & 106 & 321 \\
%   \hline
%   \textbf{Japanese} & 53 & 83 & 60 & 196 \\
%   \hline
%   \textbf{East Asian} & 45 & 73 & 46 & 164 \\  
%   \hline
%   \textbf{Nordic} & 32 & 50 & 54 & 136 \\
%   \hline
%   \textbf{Germanic} & 52 & 53 & 74 & 179 \\   
%   \hline
%   \textbf{Total Users} & 3951 & 6523 & 4163 & 14637 \\
%  \hline
% \end{tabular}
% \caption{Classification of users by ethnicity and political view for the Catalonia scenario.}
% \label{table:ethn pol}
% \end{center}
% \end{table}

% % countries + political
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%  \textbf{Country} & \textbf{Yes} & \textbf{No} & \textbf{Neutral} & \textbf{Total} \\ 
%  \hline
%   \textbf{ES} & 1388 & 3837 & 1347 & 6572 \\
%   \hline
%   \textbf{US} & 444 & 171 & 393 & 1008 \\
%   \hline
%   \textbf{GB} & 579 & 70 & 470 & 1119 \\
%   \hline
%   \textbf{FR} & 101 & 32 & 38 & 171 \\
%   \hline
%   \textbf{IT} & 71 & 29 & 65 & 165 \\
%   \hline
%   \textbf{NL} & 23 & 10 & 102 & 135 \\
%   \hline
%   \textbf{DE} & 51 & 20 & 54 & 125 \\  
%   \hline
%   \textbf{IE} & 39 & 8 & 50 & 97 \\
%   \hline
%   \textbf{BE} & 49 & 12 & 45 & 106 \\
%  \hline
%  \textbf{AT} & 4 & 0 & 7 & 11 \\
%   \hline
% \end{tabular}
% \caption{10 countries with the greatest number of polarized users for the Catalonia scenario.}
% \label{table:cntr pol}
% \end{center}
% \end{table}


% regions + political
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%  \textbf{Region} & \textbf{Yes} & \textbf{No} & \textbf{Neutral} & \textbf{Total} \\ 
%  \hline
%  \textbf{Andalusia} & 64 & 654 & 186 & 904 \\
%   \hline
%   \textbf{Catalonia} & 906 & 616 & 441 & 1963 \\
%  \hline
%   \textbf{Community of Madrid} & 116 & 963 & 245 & 1324 \\
%   \hline
%   \textbf{Valencian Community} & 68 & 281 & 69 & 418 \\
%   \hline
%   \textbf{Galicia} & 9 & 130 & 46 & 185 \\  
%   \hline
%   \textbf{Castille and León} & 8 & 127 & 46 & 181 \\
%   \hline
%   \textbf{Basque Country} & 33 & 105 & 46 & 184 \\
%   \hline
%   \textbf{Castilla-La Mancha} & 9 & 109 & 18 & 136 \\
%   \hline
%   \textbf{Canary Islands} & 10 & 122 & 23 & 155 \\
%   \hline
%   \textbf{Region of Murcia} & 7 & 122 & 22 & 151 \\
%  \hline
% \end{tabular}
% \caption{Classification of users by 10 autonomous community for the Catalonia scenario.}
% \label{table:reg pol}
% \end{center}
% \end{table}

% % cities + political
% \begin{table}
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%  \textbf{City} & \textbf{Yes} & \textbf{No} & \textbf{Neutral} & \textbf{Total} \\ 
%  \hline
%  \textbf{Madrid} & 113 & 792 & 214 & 1119 \\
%   \hline
%   \textbf{Barcelona} & 432 & 426 & 281 & 1139 \\
%   \hline
%   \textbf{Seville} & 25 & 193 & 53 & 271 \\
%   \hline
%   \textbf{Valencia} & 30 & 121 & 28 & 179 \\
%   \hline
%   \textbf{Las Palmas} & 3 & 39 & 10 & 52 \\  
%   \hline
%   \textbf{Málaga} & 9 & 86 & 23 & 118 \\
%   \hline
%   \textbf{Granada} & 4 & 48 & 19 & 71 \\
%   \hline
%   \textbf{Murcia} & 5 & 78 & 16 & 99 \\
%  \hline
%  \textbf{Bilbao} & 3 & 43 & 19 & 65 \\
%   \hline
%  \textbf{Zaragoza} & 8 & 47 & 10 & 65 \\
%   \hline
% \end{tabular}
% \caption{Classification of users by 10 cities in Spain for the Catalonia scenario.}
% \label{table:city pol}
% \end{center}
% \end{table}
